Understanding and Improving Information Transfer in Multi-Task Learning

We investigate multi-task learning approaches that use a shared feature representation for all tasks. To better understand the transfer of task information, we study an architecture with a shared module for all tasks and a separate output module for each task. We study the theory of this setting on linear and ReLU-activated models. Our key observation is that whether or not tasks' data are well-aligned can significantly affect the performance of multi-task learning. We show that misalignment between task data can cause negative transfer (or hurt performance) and provide sufficient conditions for positive transfer. Inspired by the theoretical insights, we show that aligning tasks' embedding layers leads to performance gains for multi-task training and transfer learning on the GLUE benchmark and sentiment analysis tasks; for example, we obtain a 2.35% GLUE score average improvement on 5 GLUE tasks over BERT-LARGE using our alignment method. We also design an SVD-based task reweighting scheme and show that it improves the robustness of multi-task training on a multi-label image dataset.

==> setup.tex <==
\section{Modeling Setup and Related Work}\label{sec_prelim}

There are $k$ tasks. Each task consists of a data matrix $X_i\in \real^{m_i \times d}$ and a label vector $y_i \in \real^{m_i}$, for $1 \le i \le k$.
Here we assume that all the tasks have the same input dimension.
This is commonly satisfied in applications of MTL (e.g. images with the same formats, texts where every word is represented by word vectors with the same dimensions).
\begin{align}
  \min f(A_1, A_2, \dots, A_k; B) = \sum_{i=1}^k L\Bracket{g_B(X_i) A_i, y_i}. \label{eq_mtl}
\end{align}
Here $B \in \real^{d \times H}$ is the shared module, $A_i \in \real^{H}$ is a linear output layer and $L(\cdot)$ denotes a monotone loss function.
The encoding function $g_B: \real^d \rightarrow \real$ is applied on each row of $X_i$ and depends on the shared weights $B$.
It is worth pointing out that each data point is treated equally in the above objective, whether they are from the same task or not.
This model setup is a simple abstraction of the MTL architecture (cf. \cite{C97,R17}), where the shared module $B$ provides a universal representation (e.g. an LSTM for encoding sentences or a CNN for encoding images) for different task data and each task specific module $A_i$ is optimized for task specific output.
We focus on linear and non-linear functions of $g(\cdot)$ as follows.

{\it The single task linear model:} We assume that the label vector comes from a linear model:
\begin{align*}
  y_i = X_i \theta_i + \varepsilon_i.%
\end{align*}
Each row of $X_i$ is drawn independently from a fixed distribution whose covariance is denoted by $\Sigma$ in expectation.
And every entry of the noise vector $\varepsilon_i$ follows the normal distribution with mean $0$ and variance $\sigma_i^2$.
We focus on the setting where $\Sigma$ has full rank $d$.
Hence $\theta_i$ is the unique solution provided with sufficiently many data for each task. %
Note that this corresponds to a standard setting for studying linear regression (a.k.a. the realizable setting, \cite{ELS05,HMRT19}).

{\it The ReLU model:} Denote by $\relu(x) = \max(x, 0)$ for any $x \in \real$.
We will also consider a non-linear model where the label vector comes through the ReLU activation function:
\begin{align*}
  y_i = a_i \cdot \relu(X_i \theta_i, 0) + \varepsilon_i.%
\end{align*}
It's worth mentioning that our results will apply to other non-linear functions such as leaky ReLU with bounded Lipschitz constant.

{\bf Problem statement.} Under the modeling setup, our goal is to analyze \eqref{eq_mtl} on the linear and the ReLU model to identify the quantitative factors (which may depend on the task data and the model) that affect the performance of the MTL problem.
In particular, for the linear setting, the function $g_B(X_i)$ maps to $X_i$. And for the ReLU setting, $g_B(X_i) = \relu(X_iB)$.
We will focus on analyzing regression tasks under the mean squared loss. Later on we will also validate our results on classification tasks or mixtures of regression and classification tasks. %

Before proceeding, we state the following Proposition which shows that the quality of the subspace $B$ in \eqref{eq_mtl} determines the performance of MTL. The proof and its extension involving other losses and labels can be found in Appendix \ref{append_prelim}.
\begin{proposition}\label{prop_subspace}
  In the optimum of $f(\cdot)$, each $A_i$ selects the vector $v$ within the column span of $g_B(X_i)$ to minimize $L(v, y_i)$.
  As a corollary, in the linear setting, the optimal $B$ can be achieved at a rotation matrix $B^{\star}\subseteq \real^{d\times H}$ by maximizing
  $\sum_{i=1}^k \inner{B (B^{\top}X_i^{\top}X_i B)^{\dagger} B^{\top}}{X_i^{\top}y_i y_i^{\top} X_i}.$ 
\end{proposition}


\subsection{Related Work}
There has been a large body of recent work on using the multi-task learning approach to train deep neural networks.
\cite{Glue18,Superglue19} provide the GLUE and SuperGLUE benchmarks which contain a collection of NLP tasks.
The authors show evidence that the multi-task learning approach yields superior performance than its counterpart of training a separate model per task.
\cite{MTDNN19} and their follow-up work \cite{LHCG19} obtain state of the art results on the GLUE benchmark, which inspired our study of an abstraction of the MTL model.
\cite{MKXS18} suggest a universal representation of all tasks as question answering over a context.

Of particular relevance to this work are those that develop analytical understanding of MTL and task mixing methods.
\cite{autosem} use ideas from multi-armed bandit to come up with a method for weighting each task. Compared to their method, our SVD-based method is conceptually simpler and requires less pre-processing.
\cite{AP16} identify the phenomenon of negative transfer in MTL, i.e. co-training multiple tasks does not always improve performance.
The very recent work of \cite{LV19} experiment with a similar idea of covariance normalization on images from different domains and show how to adapt models learned from one domain to a different domain by normalizing the images.
See also \cite{MBSJ09,MSGH16,PSL15,PL17} for other related work.

Finally, due to the large body of existing work on multi-task learning, we refer the interested readers to the recent survey of \cite{R17} and related surveys on domain adaptation and transfer learning by \cite{PY09,K18,C97} for complete references.
Appendix \ref{append_related} provides further review of related work.


==> setup_exp.tex <==
\section{Experimental Setup}

\paragraph{Text classification tasks.} \todo{clean up}

\paragraph{Dataset} We use six text classification tasks to verify the MTL performance over STL including movie review sentiment (MR;~\cite{pang2005seeing}), sentence subjectivity (SUBJ;~\cite{pang2004sentimental}), customer reviews polarity (CR;~\cite{hu2004mining}), question type (TREC;~\cite{li2002learning}), opinion polarity (MPQA;~\cite{wiebe2005annotating}), and the Stanford sentiment treebank (SST;~\cite{socher2013recursive}). For each task, the goal is to categorize sentiment opinions expressed in the text where formulates as classification problems over different ratings. 

\paragraph{Setup} To verify the MTL performance over STL in text classification, we use multilayer perceptron (MLP) model where the model uses an average-pooling layer over embeddings of text, followed by a multilayer perceptron. For simplicity, we use one layer in the experiments and define the output dimension of layer of multilayer perceptron as $H$ to indicate the model capacity. For the word embeddings, we use GloVe embedding trained on Wikipedia 2014 and Gigaword 5 corpora~\footnote{http://nlp.stanford.edu/data/wordvecs/glove.6B.zip} and fine tune the embeddings during the training. To report the performance, we co-train two from six tasks over 5 random seeds and report the average performance and standard deviation.



